Blockchain Transaction Processing

A blockchain is an append-only linked-list of blocks, which is maintained at each participating node. Each block records a set of transactions and their associated metadata. Blockchain transactions act on the identical ledger data stored at each node. Blockchain was first perceived by Satoshi Nakamoto as a peer-to-peer digital-commodity (also known as crypto-currency) exchange system. Blockchains received traction due to their inherent property of immutability-once a block is accepted, it cannot be reverted.

==> transaction.tex <==
\section{Transaction Processing}
Transactions in a \bc{} system are identical to their 
traditional database counterparts. 
These transactions are issued by the clients to the 
servers of the \bc{} system~\citep{nawab2018}. 
These transactions act on the data stored on all the 
participating servers. 
In its vanilla form, a \bc{} transaction could 
be visualized as a set of {\em read / write} 
operations performed on each node of a replicated 
distributed database. 
To determine an ordering for all the incoming transactions
each \bc{} application employs a 
consensus~\citep{distsystem-maarten} protocol.

Akin to the traditional distributed systems, \bc{} 
applications also emulate some form of concurrency 
control and commitment of transactions. 
It is important to understand that each \bc{} 
application needs to maintain the client data. 
Although, the client transactions are recorded in the 
%TODO: this is not necessary and not always true
%so maybe we need to say that additionally data 
%can be stored in DB to provide efficient access,
%but any data stored in DB is a secondary copy
%this could be added as footnote
block, the data is stored in an efficient database.
%TODO: concurrency control is not same as the two-phase
%two-phase is an agreement protocol while concurrency 
%is concerned with ordering/interleaving of operations 
Concurrency control in \bc{} application alludes to 
executing (or validating) a set of transactions, 
one after another, which is in principle similar to 
two phase locking. 
%TODO: this locking comment is vague and not even 
%sure if it is accurate or relevant. Probably better
%to just remove it unless, we can formalize it properly
Interestingly, depending on the nature of the 
application, locks may or may not be required.
We state these transactions as committed, when 
they are recorded in a block, which is linked to 
the {\em longest chain}.
It is possible that at any time multiple chains 
might be existing, and hence, a consensus algorithm 
helps to prune away smaller chains~\cite{blockchain-consensus}.

%TODO: the above paragraph too many things are being 
%discussed, and there is lack of logical flow or 
%or expectation from the user standpoint.
%We probably need to break into two and focus one or two
%topics in each paragraph

















